Towards a Global CE$\nu$NS Picture

We present a general framework for extracting and interpreting the Coherent Elastic Neutrino-Nucleus Scattering (CE$\nu$NS) differential cross-section from experimental data. A generalized parametric basis, constructed from common kinematic terms recurring in generalized neutrino interaction models, is employed to numerically constrain the shape and normalization of the observed CE$\nu$NS response. The framework was applied to the COHERENT CsI and liquid argon datasets using Bayesian inference, yielding normalization constraints comparable to those reported by the Collaboration while providing additional constraints on the correlated spectral shape. A combined analysis was also performed, exploiting the complementary sensitivities of the two datasets to constrain features of the differential cross-section that are less accessible to either dataset individually. The framework has been implemented in the open-source Julia package Newtrinos.jl, which supports modular forward modeling, parallel computation, and automatic differentiation.

==> figures/cevns_form_factors.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{{figures/cevns_form_factors}.pdf}
\caption{\label{fig:cevns_form_factors} Caption for cevns_form_factors.}
\end{figure*}

==> figures/csi_fit_fig.tex <==
\begin{figure}[t]
\includegraphics[width=\linewidth]{{figures/csi_fit}.pdf}
\caption{\label{fig:csi_fit} The best-fit components of the COHERENT CsI dataset overlaid with the observed data.}
\end{figure}

==> figures/lar_fit_fig.tex <==
\begin{figure}[t]
\includegraphics[width=\linewidth]{{figures/lar_fit}.pdf}
\caption{\label{fig:lar_fit} The best-fit components of the COHERENT l-Ar dataset overlaid with the observed data.}
\end{figure}

==> figures/xsec_i_fig.tex <==
\begin{figure*}[t]
\includegraphics[width=\textwidth]{{figures/xsec_i}.pdf}
\caption{\label{fig:xsec_i} Caption for xsec_i.}
\end{figure*}

==> tables/norms_CsI.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Component} & \textbf{Prior} & \textbf{Best-fit (Helm)} & \textbf{Best-fit (Klein-Nystrand)} & \textbf{Best-fit (Symm. Fermi)} & \textbf{Global best-fit estimate} \\ \hline
CE$\nu$NS & 364.7 ± 21.8  & 333.4 ± 36.4  & 356.0 ± 37.4  & 312.5 ± 35.3  & 328.9 ± 30.9  \\ \hline
BRN       & 27.4 ± 6.7    & 31.6 ± 7.0    & 31.7 ± 6.5    & 33.2 ± 6.5    & 32.6 ± 6.6    \\ \hline
NIN       & 6.9 ± 2.5     & 8.7 ± 2.4     & 6.3 ± 2.4     & 8.1 ± 2.5     & 10.3 ± 2.4    \\ \hline
SSBkg     & 3889.0 ± 80.0 & 3825.8 ± 53.0 & 3810.5 ± 52.7 & 3826.8 ± 55.8 & 3807.8 ± 51.9 \\ \hline
Total     & 4288.0 ± 83.4 & 4199.5 ± 53.0 & 4204.5 ± 53.1 & 4180.6 ± 56.1 & 4179.5 ± 55.4 \\ \hline
\end{tabular}
\end{table}

==> tables/norms_lAr.tex <==
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Component} & \textbf{Prior} & \textbf{Best-fit (Helm)} & \textbf{Best-fit (Klein-Nystrand)} & \textbf{Best-fit (Symm. Fermi)} & \textbf{Global best-fit estimate} \\ \hline
CE$\nu$NS   & 125.9 ± 3.3    & 157.0 ± 54.9  & 188.1 ± 54.0  & 162.9 ± 52.0  & 156.0 ± 43.3  \\ \hline
BRN         & 497.0 ± 160.9  & 538.6 ± 37.6  & 540.0 ± 36.9  & 560.7 ± 35.1  & 557.9 ± 33.7  \\ \hline
Delayed BRN & 33.0 ± 27.2    & 10.9 ± 9.4    & 8.7 ± 10.1    & 13.1 ± 9.4    & 9.1 ± 9.9     \\ \hline
SSBkg       & 3152.0 ± 24.1  & 3128.3 ± 23.6 & 3129.1 ± 24.7 & 3130.5 ± 22.6 & 3118.3 ± 24.3 \\ \hline
Total       & 3807.9 ± 165.6 & 3834.9 ± 46.0 & 3865.9 ± 43.9 & 3867.3 ± 46.3 & 3841.2 ± 42.7 \\ \hline
\end{tabular}
\end{table}
